Low-Rank Matrix Factorizations with Volume-based Constraints and Regularizations

Low-rank matrix factorizations are a class of linear models widely used in various fields such as machine learning, signal processing, and data analysis. These models approximate a matrix as the product of two smaller matrices, where the left matrix captures latent features while the right matrix linearly decomposes the data based on these features. There are many ways to define what makes a component "important." Standard LRMFs, such as the truncated singular value decomposition, focus on minimizing the distance between the original matrix and its low-rank approximation. In this thesis, the notion of "importance" is closely linked to interpretability and uniqueness, which are key to obtaining reliable and meaningful results. This thesis thus focuses on volume-based constraints and regularizations designed to enhance interpretability and uniqueness. We first introduce two new volume-constrained LRMFs designed to enhance these properties. The first assumes that data points are naturally bounded (e.g., movie ratings between 1 and 5 stars) and can be explained by convex combinations of features within the same bounds, allowing them to be interpreted in the same way as the data. The second model is more general, constraining the factors to belong to convex polytopes. Then, two variants of volume-regularized LRMFs are proposed. The first minimizes the volume of the latent features, encouraging them to cluster closely together, while the second maximizes the volume of the decompositions, promoting sparse representations. Across all these models, uniqueness is achieved under the core principle that the factors must be "sufficiently scattered" within their respective feasible sets. Motivated by applications such as blind source separation and missing data imputation, this thesis also proposes efficient algorithms that make these models practical for real-world applications.

==> 50titanizedminvol.tex <==
Nonnegative matrix factorization with the minimum-volume criterion (MinVol NMF) guarantees that, under some mild and realistic conditions, the factorization has an  essentially unique solution. This result has been successfully leveraged in many applications, including topic modeling, hyperspectral image unmixing, and audio source separation. In this chapter, we propose a fast algorithm to solve MinVol NMF which is based on a recently introduced block majorization-minimization framework with extrapolation steps. We illustrate the effectiveness of our new algorithm compared to the state of the art on several real hyperspectral images and document datasets.\\

The content of this chapter is mainly extracted from

\noindent\cite{vuthanh2021inertial}~\fullcite{vuthanh2021inertial}.

\section{Introduction}

Nonnegative Matrix Factorization (NMF) has been an active field of research since the seminal paper by Lee and Seung~\cite{lee99}. The success of NMF comes from many specific applications since many types of data are  nonnegative; for example 
amplitude 
spectrograms in audio source separation, images, evaluations in recommendation systems, and documents represented by vectors of word counts; see~\cite{gillis2020book} 
and the references therein. 
Compared to other unconstrained factorization models such as PCA/SVD, NMF requires the factors to be nonnegative. This constraint naturally leads to factors that are more easily interpretable~\cite{lee99}. Nonetheless, there are two drawbacks with NMF: computability and identifiability. 

\noindent \textbf{Computability.} 
As opposed to PCA/SVD, solving NMF is NP-hard in general~\cite{vavasis2009complexity}. Hence, most NMF algorithms rely on standard non-linear optimization schemes without global optimality guarantee.  

\noindent \textbf{Identifiability.} 
NMF solutions are typically not unique, that is, they are not unique even after removing the trivial scaling and permutation ambiguities of the rank-one factors; see~\cite{xiao2019uniq} and the references therein. For NMF to have a unique solution, also known as identifiability, one needs to add additional structure to the sought solution. One way to ensure identifiability is the MinVol  criterion, which minimizes the volume of one of the factors. If the sufficiently scattered condition (SSC) is satisfied, then identifiability holds for MinVol NMF~\cite{fu15,lin15,leplat2019blind}.

Identifiability for MinVol NMF is a strong result that has been used successfully in many applications such as topic modeling and hyperspectral imaging~\cite{fu16}, and audio source separation~\cite{leplat2019blind}.  
However, MinVol NMF is computationally hard to solve. In this chapter, after introducing the considered MinVol NMF model in \Cref{titanizedminvol:sec:minvolmodel}, 
we propose a fast method to solve MinVol NMF in \Cref{titanizedminvol:sec:algoTITAN}.  
Our method is an application of a recent inertial block majorization-minimization framework called TITAN~\cite{hien20}. Experimental results on real datasets show that the proposed method performs better than the state of the art; see \Cref{titanizedminvol:sec:numexp}.

\section{Minimum-volume NMF} \label{titanizedminvol:sec:minvolmodel}
In the noiseless case, the exact NMF model is $X =  W   H $ where $X\in\mathbb{R}^{m\times n}_+$ denotes the measured data, $ W \in\mathbb{R}^{m\times r}_+$ (resp.\ $ H \in\mathbb{R}^{r\times n}_+$) denotes the left factor (resp.\ the right factor). 
The idea behind the MinVol criterion, 
 a.k.a.\ Craig's belief~\cite{craig94}, is that the convex hull spanned by the columns of $ W $, denoted $\conv( W )$,  should embrace all the data points as tightly as possible. In the absence of noise, MinVol NMF is  formulated as follows 
 \begin{mini!}|s|
{ W, H }
{\det(W^\top  W )}{}{}
\addConstraint{X =  W  H}
\addConstraint{H\geq 0,~W \geq0,}{~e^\top H =e^\top,\label{titanizedminvol:const:volmin1}}
\end{mini!} 
where %$ 0 $ is a matrix of appropriate size containing only zeros and 
$ e $ is a vector of appropriate size containing only ones. The constraint~\eqref{titanizedminvol:const:volmin1} ensures that every data point lies within the convex hull spanned by the columns of $  W  $, that is, 
\mbox{$X(:,j) \in \conv( W )$} for all $j$. 
%It also prevents $  W  $ from going to $ 0 $.
The volume of the convex hull of $  W  $ and the origin in the subspace span by columns of $ W $, is proportional to $\det( W^\top W )$; see for example~\cite{fu15}.  
Under the sufficiently scattered conditions (SSC), which requires the columns of $X$ to be sufficiently spread within $\conv( W )$ or, equivalently, that $ H $ is sufficiently sparse, MinVol NMF has an essentially unique solution~\cite{fu15, lin15}. 
A drawback of \eqref{titanizedminvol:const:volmin1} is that it requires the entries in each column of $ H $ to sum to one, which is not without loss of generality: it imposes that the columns of $X$ belong to the convex hull of the columns of $ W $ as opposed to the conical hull when the equality constraints of \eqref{titanizedminvol:const:volmin1} are absent; see for example~\cite[Chapter 4]{gillis2020book}.  %\hien{(Hien: should we explain a little bit more why this assumption is not w.l.o.g or cite a paper that explains why?). 

It was recently shown that the same model where the constraint $e^\top H =e^\top$ is replaced with 
$e^\top W =e^\top$ retains identifiability~\cite{leplat2019blind}. 
The  sum-to-one constraint on the columns of $ W $, that is, $e^\top W =e^\top$, can be assumed w.l.o.g.\ via the scaling ambiguity of the rank-one factors $ W (:,k)  H (k,:)$ in any NMF decomposition. 
Moreover, the model with the constraint on $ W $  was shown to be numerically much more stable as it makes $ W $ better conditioned which is important because computing the derivative of $\det( W^\top W )$ requires computing the inverse of $ W^\top W $.  
We refer the interested reader to~\cite[Chapter 4.3.3]{gillis2020book} for a discussion on these models. 

In the presence of noise, MinVol NMF is typically formulated via penalization. In this chapter, we consider the following MinVol NMF model 
\begin{mini}|s|
	{ W,H }
	{\frac{1}{2}\left\|X- W  H \right\|^2_F+\frac{\lambda}{2}\logdet(W^\top W +\delta I)\label{titanizedminvol:eq:ourvolmin}}{}{}
	\addConstraint{ H \geq 0,~W \geq0,}{~e^\top W =e^\top,}
\end{mini} 
where 
$\|\,.\,\|_F$ is the Frobenius norm, 
$\lambda>0$ is a parameter balancing the two terms in the objective function, 
$  I $ is the $ r\times r $ identity matrix, and  $ \delta  > 0$ is a small parameter that prevents $ \logdet( W^\top W  ) $ from going to $-\infty$ if $  W  $ is rank deficient~\cite{leplat19}. 
The use of the logarithm of the determinant is  less sensible to very disparate singular values of $  W  $, leading to better practical performances~\cite{fu16,ang19}. 

\noindent \textbf{Applications.} In hyperspectral unmixing (HU), each column of $X$ contains the spectral reflectance of a pixel, each row of $X$ corresponds to the reflectance of a spectral band among all pixels, each column of $ W $ is the spectral signature of an endmember (a pure material in the image), and each column of $ H $ contains the proportion of each identified pure material in the corresponding pixel; see~\cite{bioucas2012hyperspectral}. Geometrically, the MinVol NMF in \eqref{titanizedminvol:eq:ourvolmin} applied to HU consists of finding endmembers such that the convex hull spanned by them and the origin embraces as tightly as possible every pixel in $X$. This is the so-called Craig's belief~\cite{craig94}. %when $X$ is normalized with the $\pmb{l}_\infty$-norm. 
In document classification, $X$ is a word-by-document matrix so that the columns of $ W $ correspond to topics (that is, set of words found simultaneously in several documents) while the columns of $ H $ allow to assign each documents to the topics it discusses~\cite{fu16}.  

%This behaves well with the additive $ \delta I $ which, had $  W  $ been rank deficient, would prevent the logarithm from going to minus infinity.

%The above MinVol NMF model has been shown to be particularly effective for blind hyperspectral unmixing~\cite{}. 
%The measure of the volume $ \vol( W ) = \det( W^\top W +\delta I)$. Adding $ \delta I $, where, prevents  %Let us note also that instead of enforcing $ \conv( H ) \subseteq \conv( I)$, in \Cref{titanizedminvol:const:volmin} we are enforcing $ \conv( W ) \subseteq \conv( I)$. There are several reason for this change of constraint : (i) the importance of each column of $  W  $ is more balanced, leading to a better conditioned $  W  $ and preventing $ \vol( W ) $ from being correlated to only a subset of columns of $  W  $ (ii) the constraint $ e^\top H =e^\top $ is not compatible with data points that are equal to a column of $  W  $ up to a scaling factor different than one e.g. in a multispectral scenario, if there are pixels of grass in the shadow and grass in the light, one of the two kinds can not be correctly unmixed (except if there is a zero column in $  W  $).

%$\Delta^m = \{ x\in\mathbb{R}^m~|~x \geq 0,~e^\top x=1 \}$.

\section{TITANized MinVol NMF} \label{titanizedminvol:sec:algoTITAN} 

%Our proposed VolMin consists of solving~\Cref{titanizedminvol:eq:ourvolmin}, where $ \|\,.\,\|_F $ is the Frobenius norm and  quantifies the weight of the VolMin regularization on the cost function. Let us note that instead of using directly $ \det( W^\top W +\delta I) $ as a penalization for the volume, the logarithm of this value is used as a volume penalization. 

As far as we know, all algorithms for MinVol NMF rely on two-block coordinate descent methods that update each block ($ W $ or $ H $) by using some outer  optimization algorithm to solve the subproblems formed by restricting the MinVol NMF problem to each block. %optimizing over the block variables $ W $ and $ H $ separately. 
For example, the state-of-the-art method from~\cite{leplat19} uses Nesterov fast gradient method to update each factor matrix, one at a time. 

Our proposed algorithm for~\eqref{titanizedminvol:eq:ourvolmin} will be based on the TITAN framework from~\cite{hien20}. TITAN is an inertial block majorization minimization framework for nonsmooth nonconvex optimization. It updates one block at a time while fixing the values of the other blocks, as previous MinVol NMF algorithms. 
In order to update a block, TITAN chooses a block surrogate function for the corresponding objective function (a.k.a.\ a majorizer), embeds an inertial term to this surrogate function and then minimizes the obtained inertial surrogate function. When a Lipschitz gradient surrogate is used, TITAN reduces to the Nesterov-type accelerated gradient descent step for each block of variables \cite[Section 4.2]{hien20}.
The difference of TITAN compared to previous MinVol NMF algorithms is threefold: 
\begin{enumerate} 

\item The inertial force (also known as the extrapolation, or momentum) is used between block updates. This is a crucial aspect that will make our proposed algorithm faster: when we start the update of a block of variables (here, $ W $ or $ H $), we can use the inertial force (using the previous iterate)  although the other blocks have been updated in the meantime.  
\item TITAN allows to update the surrogate after each update of $ W $ and $ H $, which was not possible with the algorithm from~\cite{leplat19} because it applied fast gradient from convex optimization on a fixed surrogate.  

\item  It has subsequential convergence guarantee, that is, every limit point of the generated sequence is a stationary point of Problem~\eqref{titanizedminvol:eq:ourvolmin}. Note that the state-of-the-art algorithm from~\cite{leplat19} does not have convergence guarantees.
\end{enumerate} 
%\item It has strong convergence guarantees, namely \ngc{give a bit more information, Hien?}. 
%\ngi{For example, the state-of-the-art algorithm that uses Nesterov fast gradient method alternatively to update $ W $ and $ H $ does not have convergence guarantees. }


%In particular and as many other NMF algorithms, our optimization process is applied in a two blocks scheme, meaning that $  W  $ will be updated while $  H  $ will be fixed, and vice-versa. 

\noindent \textbf{Remark.} 
The block prox-linear (BPL) method from~\cite{Xu2017} can be used to solve~\eqref{titanizedminvol:eq:ourvolmin} since the block functions in $ W \mapsto \frac12\|X- W  H \|^2_F$ and in $ H \mapsto \frac12\|X- W  H \|^2_F$ 
have Lipschitz continuous gradients. 
However, BPL applies extrapolation to the Lipschitz gradient surrogate of these block functions and requires to compute the proximal point of the regularizer $\frac{\lambda}{2}\logdet( W^\top W +\delta I)$, which does not have a closed form. 
In contrast, TITAN applies extrapolation to the surrogate function of $ W \mapsto f( W , H )$ with a surrogate function for the regularizer $\frac{\lambda}{2}\logdet( W^\top W +\delta I)$  (see \Cref{titanizedminvol:sec:surrogateW}). This allows TITAN  to have closed-form solutions for the subproblems, an acceleration effect, and convergence guarantee.   
%In the line of alternating exptrapolation algorithms, it is worth mentioning  However, BPL applies extrapolation to the Lipschitz gradient surrogate of these block functions and requires to compute the proximal point of the regularizer $\frac{\lambda}{2}\logdet( W^\top W +\delta I)$, which does not have a closed-form solution. In contrast, TITAN apply extrapolation to the surrogate function of $ W \mapsto f( W , H )$ that also employs a surrogate function for the regularizer $\frac{\lambda}{2}\logdet( W^\top W +\delta I)$  (see details in \Cref{titanizedminvol:sec:surrogateW}). By this way, TITAN not only has closed-form solutions for its subproblems, but also obtains acceleration effect.

\subsection{Surrogate functions} \label{titanizedminvol:sec:surrogates}
An important step of TITAN is to define a surrogate function for each block of variables. 
These surrogate functions are upper approximation of the objective function at the current iterate. %In particular, we choose to use Lipschitz gradient surrogates. 
Denote 
\[f( W ,  H ) = \frac{1}{2}\left\|X- W  H \right\|^2_F+\frac{\lambda}{2}\logdet( W^\top W +\delta I)\] and suppose we are cyclically updating $( W , H )$. Let us denote
%also know as a majorizer, is a function that is larger th 
%Let us describe our method. First, let us focus on the majorization aspect by 
 $u_{W_k}( W )$ the surrogate function of $ W \mapsto f( W ,H_k) $ to update $W_k$, that is,  %$f( W , H )$ at $W_k$ such that  
\begin{equation}
	f( W ,H_k) \leq u_{W_k}( W ) 
	\; 
	\text{ for all } 
	\; 
	 W  \in \mathcal{X}_W , 
\end{equation} 
where $ u_{W_k}(W_k) =f(W_k,H_k)$ and $\mathcal{X}_W $ is the feasible domain of $  W  $. Similarly, let us denote $u_{H_k}( H )$ the surrogate function of $ H \mapsto f(W_{k+1}, H )$ to update $H_k$, that is 
\begin{equation}
	f(W_{k+1}, H )\leq u_{H_k}( H ) 
	\; 
	\text{ for all } 
	\; 
	 H  \in \mathcal{X}_H ,  
\end{equation}
where $u_{H_k}(H_k) =f(W_{k+1},H_k)$ and $\mathcal{X}_H $ is the feasible domain of $  H  $. \\

\subsubsection{Surrogate function and update of  $ W $} 
\label{titanizedminvol:sec:surrogateW}
%Let us suppose that $  H  $ is fixed. 

Denote $ A =  W^\top W +\delta I,~B_k = W_k^\top W_k+\delta I $ and $ P_k = (B_k)^{-1}$. Since $ \logdet $ is concave, its first-order Taylor expansion around $B_k$ leads to $\logdet(A)\leq \logdet(B_k) + \langle (B_k)^{-1},A-B_k \rangle$. Hence,
\begin{equation}
f( W ,H_k)\leq \widetilde{f}_{W_k}( W )
:=\frac{1}{2}\left\|X- W H_k\right\|^2_F + \frac{\lambda}{2}\langle P_k, W^\top W  \rangle + C_1,
\label{titanizedminvol:eq:majorW}
\end{equation}
where $C_1$ is a constant independent of $ W $. %(Hien: we don't need to use the subscript $C_W$ since it may make cause some misunderstanding that $C_W$ depends on $W$)
%$ C_{ W } $ is a constant {\color{orange}in-?}depending {\color{orange}on} $  W  $. %However, $\tilde{f}_{W_k}$ is still hard to minimize. 
Note that the gradient of $ W \mapsto\widetilde{f}_{W_k}( W )$, being equal to \[( W H_k-X)H_k^\top+\lambda  W P_k,\] is $ L^k_W  $-Lipschitz continuous with $ L^k_W =\|H_kH_k^\top+\lambda P_k\|_2 $. Hence, from~\eqref{titanizedminvol:eq:majorW} and the descent lemma (see \cite[Section 2.1]{Nesterov2018}),  %can use the descent Lemma again to choose our Lipschitz gradient surrogate:
\begin{equation}
f( W ,H_k) \leq u_{W_k}( W ) := \langle\nabla \widetilde{f}_{W_k}(W_k), W \rangle + \frac{L^k_W }{2}\| W -W_k\|^2_F + C_2, 
\label{titanizedminvol:eq:surrogateforW}
\end{equation}
where $C_2$ is a constant depending on $W_k$. 
% {\color{orange}(Andersen: independent on W? if dependent why this term disappear in (7)?) } \hien{Andersen: it depends on $W_k$ but it is a constant independent of $W$.}
% \ngc{depending on $W_k$?} % different than $C_{ W }$ in \Cref{titanizedminvol:eq:majorW}. 
We %will
use the surrogate $u_{W_k}( W ) $ defined in~\eqref{titanizedminvol:eq:surrogateforW} to update $W_k$. As TITAN recovers Nesterov-type acceleration for the update of each block of variables~\cite[Section 4.2]{hien20}, 
we have the following update for $ W $:   
\begin{equation}
\label{titanizedminvol:eq:updateW}
\begin{split}
 W_{k+1}   & = \argmin_{ W \in\mathcal{X}_W } \langle\nabla \widetilde{f}_{W_k}(\overbar{W_k}), W \rangle + \frac{L^k_W }{2}\| W -\overbar{W_k}\|^2_F, \\
            & = \mathscr{P}\left( \overbar{W_k} + \frac{(X-\overbar{W_k}H_k)H_k^\top-\lambda\overbar{W_k}P}{L_W^k} \right),
\end{split}
\end{equation}
where $\mathscr{P}$ performs column wise projections onto the unit simplex as in~\cite{condat2016} in order to satisfy the constraint on $ W $ in \eqref{titanizedminvol:eq:ourvolmin}, and where $\overbar{W_k}$ is an extrapolated point, that is, the current point $W_k$ plus some momentum,
\begin{equation}
    \overbar{W_k} = W_k + \beta_{ W }^{k}(W_k-W_{k-1}),
\end{equation}
where the extrapolation parameter $\beta_{ W }^{k}$ is chosen as follows 
\begin{equation}
    \label{titanizedminvol:eq:betaW}
\beta_{ W }^{k} = \min\left[~ \dfrac{\alpha_k-1}{\alpha_{k+1}} ,0.9999\sqrt{\dfrac{L_W^{k-1}}{L_W^{k}}} ~\right],  
\end{equation}
$\alpha_0=1$, $\alpha_k=(1+\sqrt{1+4 \alpha_{k-1}^2})/2$. This choice of parameter satisfies the conditions to have a subsequential convergence of TITAN, see \Cref{titanizedminvol:sec:convergence}.  %according to~\cite[Section 6.1]{hien20}. 
% The index here is $\beta_{ W }^{k}$ since we are at the $k$ iterate. 
%A common choice for $\alpha_0$ would be $\alpha_0=1$.


% {\color{orange} (Andersen: if I am in charge, I will greatly simplify this subsection on H and by using " symmetry", and say "by symmetry, the update of H is blablablabla.")} \ngc{This is in fact an option. If we have enough space, this is not necessary.} 

\subsubsection{Surrogate function and update of  $ H $} \label{titanizedminvol:sec:surrogateH}
Since
\[
\nabla_H  f(W_{k+1}, H )=W_{k+1}^\top(W_{k+1} H -X),
\]
the gradient of $ f $ according to $  H  $ is $L_H^{k}$-Lipschitz 
% \hien{(Hien: Note that for cyclic update rule, although $ W $ was updated to $k+1$ but we are still at iteration $k$ to update $ H $, so the index of $L_H $ is still $k$)} 
continuous with $L_H^{k}=\|W_{k+1}^\top W_{k+1}\|_2$. Hence, we use the following Lipschitz gradient surrogate to update $H_k$: 
\begin{equation}
	u_{H_k}( H ) = \langle\nabla_H  f(W_{k+1},H_k), H \rangle + \frac{L^k_H }{2}\| H -H_k\|^2_F +C_3,
\label{titanizedminvol:eq:surrogateH}
\end{equation}
where $ C_3 $ is a constant depending on $ H_k $. 
%{\color{orange} (Andersen: again, it should be "independent on H" right? if it is dependnet then why it disappear in the update below?)}
% \ngc{It should depend on $H_k$, right?} 
We derive our update rule for $ H $ by minimizing the surrogate function from \Cref{titanizedminvol:eq:surrogateH} embedded with extrapolation,
\begin{equation}
	\label{titanizedminvol:eq:minsurrogateH}
\begin{split}
	H_{k+1}    & = \argmin_{ H \in\mathcal{X}_H} \langle\nabla_H  f(W_{k+1},\overbar{H_k}), H \rangle + \frac{L^k_H }{2}\| H -\overbar{H_k}\|^2_F, \\
	& = \left[\overbar{ H }_k+\frac{1}{L_H^{k}}W_{k+1}^\top(X-W_{k+1}\overbar{ H }_k)  \right]_+,
\end{split}
\end{equation}
where $[\,.\,]_+$ denotes the projector setting all negative values to zero, and 
%where
$\overbar{H_k}$ is the extrapolated $H_k$: 
\begin{equation}
    \overbar{H_k}=H_k+\beta^{k}_H (H_k - H_{k-1}),
\end{equation}
 where, as for the update of $ W $, % in \Cref{titanizedminvol:sec:surrogateW},
 \begin{equation}
     \beta_{ H }^{k} = \min\left[~ \dfrac{\alpha_k-1}{\alpha_{k+1}} ,0.9999\sqrt{ \dfrac{L_H^{k-1}}{L_H^{k}}} ~\right].
 \end{equation}

\subsection{Algorithm} \label{titanizedminvol:sec:algodesc}
Note that the update of $ W $ in~\eqref{titanizedminvol:eq:updateW} and $ H $ in~\eqref{titanizedminvol:eq:minsurrogateH} was described when the cyclic update rule is applied. Since  TITAN also allows the essentially cyclic rule~\cite[Section 5]{hien20}, we can update $ W $ several times before switching updating $ H $, and vice versa. 
This leads to our proposed method TITANized MinVol, see \Cref{titanizedminvol:algo:ourmethod} for the pseudocode.
The stopping criteria in \cref{titanizedminvol:algo:stopcritW,titanizedminvol:algo:stopcritH} are the same as in \cite{leplat19}. The way $\lambda$ and $\delta$ are computed is also identical to~\cite{leplat19}. 
Let us mention that technically the main difference with \cite{leplat19} resides in how the extrapolation is embedded. In \cite{leplat19} the Nesterov sequence is restarted and evolves in each inner loop to solve each subproblem corresponding to each block. In our algorithm, the extrapolation parameter $\beta_W $ (and $\beta_H $) for updating each block $ W $ (and $ H $) is updated continuously without restarting.
It means we are accelerating the global convergence of the sequences rather than trying to accelerate the convergence for the subproblems. Moreover, TITAN allows to update the surrogate function at each step, while the algorithm from \cite{leplat19} can only update it before each subproblem is solved, as it relies on Nesterov's acceleration for convex optimization.


\begin{algorithm}{thb!}
    \caption{TITANized MinVol}
    \DontPrintSemicolon
    \KwIn{$W_0,H_0,\lambda,\delta$}
    $\alpha_1=1$, $\alpha_2=1$, $W_{old}=W_0,H_{old}=H_0$, $L_H^{prev}=\|W_{0}^\top W_{0}\|_2$, $L_W^{prev}=\|H_{0} H^\top_{0}+\lambda (W_{0}^\top W_{0}+\delta I)^{-1}\|_2$\;
    \KwOut{$W,H$}
    \While{stopping criteria not satisfied}{
        \While{stopping criteria not satisfied\label{titanizedminvol:algo:stopcritW}}{
            $\alpha_{0}=\alpha_1, \alpha_1=(1+\sqrt{1+4\alpha_0^2})/2$\;
            $ P \leftarrow ( W^\top W +\delta I)^{-1} $\;
            $L_W  \leftarrow\| H  H^\top+\lambda P\|_2 $\;
            $\beta_{ W }=\min\left[~(\alpha_0-1)/\alpha_{1},0.9999\sqrt{L_W^{prev}/L_W } ~\right] $\;
            $\overbar{ W }\leftarrow W +\beta_{ W }( W -W_{old}) $\;
            $W_{old}\leftarrow  W $\;
            $ W  \leftarrow \mathscr{P}\left[\overbar{ W }+\frac{(X H^\top-\overbar{ W }( H  H^\top+\lambda P))}{L_W }\right]$\;
            $ L_W^{prev} \leftarrow L_W $\;
        }
        $ L_H  \leftarrow \| W^\top W \|_2 $\;
        \While{stopping criteria not satisfied\label{titanizedminvol:algo:stopcritH}}{ 
            $\alpha_{0}=\alpha_2, \alpha_2=(1+\sqrt{1+4\alpha_0^2})/2$\;
            $ \beta_{ H }=\min\left[~(\alpha_0-1)/\alpha_{2},0.9999\sqrt{L_H^{prev}/L_H } ~\right] $\;
            $ \overbar{ H } \leftarrow  H +\beta_{ H }( H -H_{old}) $\;
            $H_{old}\leftarrow  H $\;
            $  H  \leftarrow \left[\overbar{ H }+\frac{ W^\top(X- W \overbar{ H }) }{L_H } \right]_+ $\;
            $L_H^{prev} \leftarrow L_H $\;
        }
    }
    \label{titanizedminvol:algo:ourmethod}
    \end{algorithm}

\subsection{Convergence guarantee} \label{titanizedminvol:sec:convergence}

%To the best of our knowledge, subsequential convergence with acceleration steps has not been studied for block successive upper-bound minimization (BSUM) except in~\cite{hien20}. 

In order to have a convergence guarantee, TITAN requires the update of each block to satisfy the nearly sufficiently decreasing property (NSDP), see \cite[Section 2]{hien20}.  
By \cite[Section 4.2.1]{hien20}, the update for $ H $ of TITANized MinVol satisfies the NSDP condition since it uses a Lipschitz gradient surrogate for $ H \mapsto f( W , H )$ combined with the Nesterov-type extrapolation; and the bounds of the extrapolation parameters in the update of $ H $ are derived similarly as in \cite[Section 6.1]{hien20}. However, it is important noting that the update for $ W $ of TITANized MinVol does not directly use a Lipschitz gradient surrogate for $ W \mapsto f( W , H )$. We thus need to verify NSDP condition for  the update of $ W $ by another method that is presented in the following.  

The function $u_{W_k}( W )$ is a Lipschitz gradient surrogate of $\tilde f_{W_k}( W ) $, and we apply the Nesterov-type extrapolation to obtain the update in \eqref{titanizedminvol:eq:updateW}. Note that the feasible set of $ W $ is convex.  Hence, it follows from \cite[Remark 4.1]{hien20} that 
\begin{equation}
\label{titanizedminvol:eq:NSDP1}
    \tilde f_{W_k}(W_k) + \frac{L_{ W }^k (\beta_{ W }^k)^2}{2}\|W_k-W_{k-1}\|^2_F 
    \geq
    \tilde f_{W_k}(W_{k+1}) + \frac{L_{ W }^k}{2}\|W_{k+1}-W_k\|^2_F.
\end{equation}
Furthermore, we note that $ \tilde f_{W_k}(W_k)=f(W_k,H_k)$, and $ \tilde f_{W_k}(W_{k+1}) \geq f(W_{k+1},H_k)$. Therefore, from~\eqref{titanizedminvol:eq:NSDP1} we have 
\begin{equation}
    f(W_k,H_k) + \frac{L_{ W }^k (\beta_{ W }^k)^2}{2}\|W_k-W_{k-1}\|^2_F 
    \geq
    f(W_{k+1},H_k) + \frac{L_{ W }^k}{2}\|W_{k+1}-W_k\|^2_F,
\end{equation}
which is the required NSDP condition of TITAN. Consequently, the choice of $\beta_{ W }^k$ in~\eqref{titanizedminvol:eq:betaW}  satisfy the required condition to guarantee subsequential convergence~\cite[Proposition 3.1]{hien20}.  

On the other hand, we note that the error function $ W  \mapsto err_1( W ):= u_{W_k}( W  )-f( W ,H_k )$ is continuously differentiable and  $\nabla_{ W } err_1(W_k )=0$; similarly for the error function $ H  \mapsto err_2( H ):= u_{H_k}( H  )-f(W_{k+1}, H  )$. Hence, it follows from \cite[Lemma 2.3]{hien20} that the Assumption 2.2 in \cite{hien20} is satisfied. Applying \cite[Theorem 3.2]{hien20}, we conclude that every limit point of the generated sequence is a stationary point of Problem~\eqref{titanizedminvol:eq:ourvolmin}. It is worth noting that as TITANized MinVol does not apply restarting step, \cite[Theorem 3.5]{hien20} for a global convergence is not applicable.      %\ovc{define global convergence}, TITAN needs four assumptions to hold. Since an exhaustive proof is beyond the scope of this paper, we quickly give here some ideas to prove that our algorithm meets the requirements for global convergence in TITAN framework.

%\begin{enumerate}
 %   \item \textbf{Nearly sufficient decrease property:} If we focus on $ W $, the surrogate function $u_{W_k}$ and the extrapolation must generate a sequence $(W_k)_{k\in\mathds{N}}$ such that
%\begin{multline}
%    \forall k \in \mathds{N},
 %   f(W_k,H_k) + \frac{\gamma_{ W }^{(W_k,H_k)}}{2}\|W_k-W_{k-1}\|^2_F \\
 %   \geq
 %   f(W_{k+1},H_k) + \frac{\eta_{ H }^{(W_k,H_k)}}{2}\|W_{k+1}-W_k\|^2_F
%\label{titanizedminvol:eq:nsdp}
%\end{multline}
%where $\gamma_{ W }^{(W_k,H_k)}$ and $\eta_{ H }^{(W_k,H_k)}$ depends on the extrapolation parameters and $u_{W_k}$. Since we chose to use Lipschitz gradient surrogates, $u_{W_k}$ is $L_W^k$ strongly convex. Then we can derive $\gamma_{ W }^{(W_k,H_k)}$ and $\eta_{ H }^{(W_k,H_k)}$ using~\cite[Theorem 2.7]{hien20} such that \Cref{titanizedminvol:eq:nsdp} holds. The same reasoning can be applied to $ H $. 
 %   \item \textbf{Boundedness of subgradient:}
  %  \item \textbf{Kurdyka- Lojasiewicz property:} \ovc{I looked for it but still don't quite understand... }
  %  \item \textbf{A continuous condition:}
%\end{enumerate}

\section{Numerical Experiments} \label{titanizedminvol:sec:numexp}

In this section we compare TITANized MinVol to~\cite{leplat19}, an accelerated version of the method from~\cite{fu16} (for $p=2$), on two NMF applications: hyperspectral unmixing and document clustering, which are dense and sparse datasets, respectively. All tests are performed on MATLAB R2018a, on a PC with an Intel® Core™ i7 6700HQ and 24 GB RAM. The code is available on an online repository\footnote{\url{https://gitlab.com/vuthanho/titanized-minvol}}.

% The hyperspectral datasets are the following: Urban (307 by 307 with 162 spectral bands), Indian Pines (145 by 145 with 200 spectral bands), Pavia University (610 by 340 with 103 spectral bands), San Diego (400 by 400 with 158 spectral bands) and Terrain (500 by 307 with 166 spectral bands). The document datasets are the following: 20 News (61188 words and 7505 documents), Sports (14870 words and 8580 documents) and Reviews (18483 words and 4069 documents). 
The datasets used are shown in \Cref{titanizedminvol:tab:datasets}. For each data set, each algorithm is launched with the same random initializations, for the same amount of CPU time. In order to derive some statistics, for both hyperspectral unmixing and document clustering, 20 random initializations are used (each entry of $ W $ and $ H $ are drawn from the uniform distribution in [0,1]).  %Experiments with a warm start with SNPA~\cite{gillis14} are not shown for the sake of concision since the same behaviors have been drawn out from experiments with a warm start or with random initializations. 
The CPU time used for each data set is adjusted manually, and corresponds to the maximum displayed value on the respective time axes in \Cref{titanizedminvol:fig:avg}; see also \Cref{titanizedminvol:tab:leadtime}.  
% \begin{table}[tbh!]
%     \centering
%     \normalsize
%     \begin{tabular}{l|c}
%         data set     & Dimensions \\ \hline\hline
%         Urban       & 307 by 307 pixels by 162 spect. bands   \\
%         Indian Pine & 145 by 145 pixels by 200 spect. bands \\
%         Pavia Univ. & 610 by 340 pixels by 103 spect. bands \\
%         San Diego   & 400 by 400 pixels by 158 spect. bands \\
%         Terrain     & 500 by 307 pixels by 166 spect. bands \\
%         20 News     & 61188 words by 7505 doc. \\
%         Sports      & 14870 words by 8580 doc. \\
%         Reviews     & 18483 words by 4069 doc. \\
%     \end{tabular}
    
%     \caption{datasets used in our experiments and their respective dimensions}
%     \label{titanizedminvol:tab:datasets}
% \end{table}

\begin{table}[thb!]
    \centering
    \normalsize
    \begin{tabular}{l||c|c|c}
        Data set     & $m$ & $n$ & $r$ \\ \hline
        Urban       & 162 & 94249 & 6   \\
        Indian Pine & 200 & 21025 & 16 \\
        Pavia Univ. & 103 & 207400 & 9 \\
        San Diego   & 158 & 160000 & 7 \\
        Terrain     & 166 & 153500 & 5 \\
        20 News     & 61188 & 7505 & 20 \\
        Sports      & 14870 & 8580 & 7 \\
        Reviews     & 18483 & 4069 & 5 \\
    \end{tabular}
    
    \caption{Datasets used in our experiments and their respective dimensions}
    \label{titanizedminvol:tab:datasets}
\end{table}

For display purposes, for each data set, we compare the average of the scaled objective functions according to time, that is, the average of  $(f( W , H )-e_{\min})/\|X\|_F$ where $e_{\min}$ is the minimum obtained error among the 20 different runs and among both methods. The results are presented in \Cref{titanizedminvol:fig:avg}. On both hyperspectral and document datasets,  TITANized MinVol converges on average faster than \cite{leplat19} except for the San Diego data set (although TITANized MinVol converges initially faster). For most tested datasets, MinVol~\cite{leplat19} cannot reach the same error as TITANized MinVol within the allocated time. 

\begin{figure}[htbp!]
\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Urban}
\tikzexternalexportnextfalse % ref with tikz externalize doesn't work together
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean urban,
% 		restrict x to domain=0:60,
		ymax=1e-4,
% 		xmax = 10,
		% xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
		legend entries={TITANized MinVol,MinVol from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_urban1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_urban2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Indian Pines}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean indian,
% 		restrict x to domain=0:60,
		ymax=1e-4,
		% xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_indian1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_indian2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\vspace{0.3cm}

\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Pavia Uni}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean paviau,
% 		restrict x to domain=0:60,
		ymax=1e-4,
% 		ymin=1e-5,
		% xlabel={time (s)},
		xtick={0,30,60,90},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_paviau1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_paviau2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{San Diego}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean sandiego,
% 		restrict x to domain=0:60,
		ymax=1e-4,
		ymin=1e-5,
		% xlabel={time (s)},
		xtick={0,40,80,120},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_sandiego1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_sandiego2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\vspace{0.3cm}

\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Terrain}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean terrain,
% 		restrict x to domain=0:60,
		ymax=1e-4,
		% xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_terrain1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_hyper/mean_terrain2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{20News}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean 20news,
% 		restrict x to domain=0:60,
		ymax=1e-3,
		% xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_20news1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_20news2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\vspace{0.3cm}

\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Reviews}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean reviews,
% 		restrict x to domain=0:60,
		ymax=1e-3,
% 		xmax=30,
		xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_reviews1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_reviews2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\captionsetup{skip=0pt}
\caption{Sports}
\begin{tikzpicture}
	\begin{semilogyaxis}[
% 		title = mean sports,
% 		restrict x to domain=0:60,
		ymax=1e-3,
% 		xmax=15,
		xlabel={time (s)},
% 		ylabel={$(f( W , H )-e_{\min})/\|X\|_F$},
		grid=major,width = \textwidth,height=4cm,cycle list name=exotic,no markers,
% 		legend entries={TITANized MinVol,VolMin from~\cite{leplat19}},
		]
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_sports1.dat};
		\addplot+[line width = 2pt]table {titanizedminvol/results_doc/mean_sports2.dat};
	\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\caption{Evolution w.r.t.\ time of the average of  $(f( W , H )-e_{\min})/\|X\|_F$ for the  different datasets.} 
\label{titanizedminvol:fig:avg}
\end{figure}

%In particular, TITANized MinVol achieves a lower error in 94 out of the 100 runs for the hyperspectral images (5 images with 20 random initialization each), and 55 out of 60 for the document datasets (3 sets of documents with 20 random initialization each). 

%Most of the time (94\% of the time for 100 tests), at the end of the dedicated CPU time, TITANized MinVol obtained the minimum error for hyperspectral unmixing. For document clustering, the difference between both compared methods is of the same order as TITANized MinVol obtained the minimum error 92\% of the time for 60 tests. 

\begin{center}
\begin{table}[thb!] 
    \begin{center} 
    \normalsize
        \begin{tabular}{l||c|c|c} 
            Data set     & Our method's & CPU time 
            & 
            Saved \\
                        & lead time (s) & 
                for~\cite{leplat19}  &  CPU time \\ 
            \hline 
            Urban       &  $ 44$  & 60 & 73\% \\ 
            Indian Pines&  $ 25$  & 30 & 83\% \\
            Pavia Univ. &  $ 68$  & 90 & 76\% \\ 
            San Diego   &  NaN    & 120 & 0\% \\ 
            Terrain     &  $ 44$  & 60 & 73\% \\ 
            20News      &  $221$  & 300 & 74\% \\ 
            Reviews     &  $ 26$  & 30 & 80\% \\ 
            Sports      &  $ 15$  & 30 & 50\% \\ 
        \end{tabular}
    \end{center} 
\caption{TITANized MinVol's lead time over MinVol~\cite{leplat19} to obtain the same minimum error.}
\label{titanizedminvol:tab:leadtime}
\end{table} 
\end{center}

\begin{center}
\begin{table}[thb!]
    \centering
    \normalsize
    \begin{tabular}{c||c|c} 
        \multirow{2}{*}{Algorithm}  & \multicolumn{2}{c}{ranking} \\ \cline{2-3}
                                    & Hyperspectral unmixing    & Document clustering \\ \hline
        TITANized MinVol                  & $( 94, 6 ) $                & $( 55, 5 )$ \\ \hline
        MinVol \cite{leplat19}     & $(  6,94 )$                 & $(  5,55 )$ 
    \end{tabular}
    \caption{Ranking among the different runs depending on the algorithm and the kind of data set}
    \label{titanizedminvol:tab:ranking}
\end{table}
\end{center}

The ranking among all the tests has been reported in~\Cref{titanizedminvol:tab:ranking}, where the $i$-th entry denotes how many times the corresponding algorithm was in the $i$-th place. We also reported in \Cref{titanizedminvol:tab:leadtime} TITANized MinVol's lead time over~\cite{leplat19} when the latter reaches its minimum error after the maximum allotted CPU time. The lead time is the time saved by TITANized MinVol to achieve the error of the method from~\cite{leplat19} using the maximum allotted CPU time. 
On average, TITANized MinVol is twice faster than \cite{leplat19}, with an average gain of CPU time above 50\%. %That said, a significant amount of CPU time could be saved by using TITANized MinVol. 

To summarize, our experimental results show that TITANized MinVol has a faster convergence speed and smaller final solutions than \cite{leplat19}. 


\section{Conclusion and Discussion}

We developed a new algorithm to solve MinVol NMF~\eqref{titanizedminvol:eq:ourvolmin} based on the inertial block majorization-minimization framework of~\cite{hien20}. This framework, under some conditions that hold for our method, guarantees subsequential convergence. Experimental results show that this acceleration strategy performs better than the state-of-the-art accelerated MinVol NMF algorithm from~\cite{leplat19}. Future works will focus on different types of acceleration such as Anderson's acceleration~\cite{anderson65}, and on different constraints on $ W $ and/or $ H $ to address some specific applications. 


==> 60minvolNMC.tex <==
Low-rank matrix approximation is a standard, yet powerful, embedding technique that can be used to tackle a broad range of problems, including the recovery of missing data. In this chapter, we focus on the performance of nonnegative matrix factorization (NMF) with minimum-volume (MinVol) regularization on the task of nonnegative data imputation. The particular choice of the MinVol regularization is justified by its interesting identifiability property and by its link with the nuclear norm. We show experimentally that MinVol NMF is a relevant model for nonnegative data recovery, especially when the recovery of a unique embedding is desired. Additionally, we introduce a new version of MinVol NMF that exhibits some promising results.

\section{Introduction}
\label{minvolnmc:sec:intro}

Given a data matrix $X\in\R^{m\times n}$, there exist many scenarios where only a few entries of $X$ are observed, e.g., in recommender systems illustrated by the famous Netflix problem~\cite{koren2009matrix}. 
Recovering these missing entries is often tackled by assuming that the fully observed data follow a certain structure. 
If the structuring assumption is meaningful, by fitting a model that follows the same structure on the observed entries, it is possible to recover the missing entries; see, e.g., ~\cite{candes2010matrix,gross2011recovering,candes2012exact}. 
The low-rank assumption is meaningful in many scenarios~\cite{udell2019big}. If $X\in\R^{m\times n}$ is low rank, we can express it as the product of two smaller matrices, $W\in\R^{m\times r}$ and $H\in\R^{r\times n}$, as $X=WH$ where $r\ll\min(m,n)$. 
Let us denote $\Omega\subseteq\{1,\dots,m\}\times\{1,\dots,n\}$ the set containing the indices of the observed entries in $X$. 
If the rank of $X$ is equal to $r$, we can look for $W\in\R^{m\times r}$ and $H\in\R^{r\times n}$ such that $X(i,j)=W(i,:)H(:,j)$ for all $(i,j)\in\Omega$. Then, for every missing entry at $(i,j)\in\overbar{\Omega}$, $X(i,j)$ can be estimated by computing $W(i,:)H(:,j)$. If $X$ is noisy and does not follow the low-rank assumption, it might still be relevant to approximate it through a low-rank structure, because low-rank matrix approximations can identify patterns in the data via the extraction of common features among data points.  

When the rank is unknown, a common tractable strategy is to minimize the nuclear norm, that is the sum of the singular values, of the estimation $\tilde{X}$ of $X$: 
% \begin{mini*}
% 	{}{\|\tilde{X}\|_*}{}{}
% 	\addConstraint{\P_\Omega(\tilde{X})}{=\P_\Omega(X),}{}
% \end{mini*}
\begin{equation*}
	\min_{\tilde{X}} \| \tilde{X} \|_*  
	\quad \text{ such that } \quad \P_\Omega(\tilde{X}) = \P_\Omega(X), 
\end{equation*}
where $\P_\Omega(Y)$ sets $Y(i,j)$ to zero if $(i,j)\notin\Omega$, or does not change it otherwise.

In this chapter, we consider the rank to be known, and our goal is not only to recover the missing entries in $X$, but also to recover the unique matrices $W$ and $H$ that generated the data $X=WH$. This could be useful in hyperspectral unmixing with missing data for instance, where the columns of $W$ are expected to be the spectral signatures of the underlying materials, and where the $j$-th column of $H$ contains the abundance in the $j$-th pixel of each extracted material. In this scenario, it is of course preferable to recover a unique set $(W,H)$. %\ngc{Mention the motivation? Some applications? e.g., hyperspectral unmixing with missing data?} 
To perform this task, it is possible to first use a data completion algorithm, and then use a constrained matrix factorization algorithm to estimate the sought factors $W$ and $H$. Here, we focus on performing both tasks together, since estimating correctly $W$ and $H$ on $\Omega$ implies a correct recovery of the missing entries in $X = WH$.
We assume that the data and the factors are nonnegative, that is, $X\geq0$, $W\geq0$ and $H\geq0$, where $\geq$ is applied element wise. In the fully observed case, estimating nonnegative $W$ and $H$ from $X$ is known as nonnegative matrix factorization (NMF)~\cite{lee1999learning}. Hence, our goal is to perform NMF with missing data while recovering a unique decomposition. To do so, minimum-volume (MinVol) NMF is a relevant option, and its performances on matrix completion have never been explored before. In this chapter, we show that when correctly tuned, MinVol NMF performs well on the matrix completion task and is also able to retrieve the true underlying factors  using only a few observed entries. 

The chapter is organized as follows. In~\Cref{minvolnmc:sec:minvolnmf}, we introduce MinVol NMF and its identifiability properties. In~\Cref{minvolnmc:sec:NMC}, we introduce the nonnegative matrix completion problem and discuss on the relevance of MinVol NMF for this problem. We also introduce a new variant of MinVol NMF. In~\Cref{minvolnmc:sec:algorithms}, we describe the algorithms used in the experiment presented in~\Cref{minvolnmc:sec:exp}. Finally, we conclude and discuss future work in~\Cref{minvolnmc:sec:conclusion}.
 

\section{minimum-volume NMF (MinVol NMF)}
\label{minvolnmc:sec:minvolnmf}

\subsection{Existing declinations of MinVol NMF}


% Like NMF, the main purpose of Minvol NMF is to explain the data with conic combinations of nonnegative features. \ngc{On ne voit pas trop d'où ça sort ce cone... il faudrait réexpliquer rapidement l'interprétation géométrique de NMF.} Distinctively, with Minvol NMF the features \ngc{what features? Il faudrait mieux présenter le problème} should enclose the data as tightly as possible, hence the expression ``minimum-volume''. Let us consider some data $X\in\R_+^{m\times n}$, in the exact case Minvol NMF consists in finding a couple of factors $(W,H)\in\R_+^{m\times r}\times\R_+^{r\times n}$ such that $X=WH$ while minimizing the volume spanned by the columns of $W$ and the origin, which is given by $\frac{1}{r!}\sqrt{\det(\Wt W)}$. 
Given a matrix $X\in\R_+^{m\times n}$ and a factorization rank $r$, in the exact case NMF consists in finding two smaller matrices $W\in\R_+^{m\times r}$ and $H\in\R_+^{r\times n}$ such that $X=WH$. Geometrically, this implies that $\cone(X)\subseteq\cone(W)$\footnote{Given $A\in\R^{m\times n}$, $\cone(A)=\{y \ | \ y=Ax\text{ for }x\in\R^n_+\}$.}. Distinctively, with MinVol NMF the cone of $W$ should enclose the cone of $X$ as tightly as possible, hence the expression ``minimum-volume''. In other words, MinVol NMF consists in finding a couple of factors $(W,H)\in\R_+^{m\times r}\times\R_+^{r\times n}$ such that $X=WH$ while minimizing the volume of the convex hull of %spanned by 
the columns of $W$ and the origin, which is given by $\frac{1}{r!}\sqrt{\det(\Wt W)}$. 
This improves the interpretability of the features (the columns of $W$) while prioritizing a unique decomposition of the data under relatively mild assumptions, that are given in~\Cref{minvolnmc:th:uniqueminvol}. Additionally, one of the factors should be constrained 
% \ngc{pas très clair ce que veut dire norm constrainted}. Without such a constraint, 
such that the scaling ambiguity between $W$ and $H$ coupled with the minimized volume does not make $W$ tend to zero at optimality. 
%Depending on the application, usual 
Identifiable MinVol NMFs typically use simplex structuring constraints, namely $W\in\Delta^{m\times r}$~\cite{leplat2019blind} or $H\in\Delta^{r\times n}$~\cite{fu2015blind} or $H^\top\in\Delta^{n\times r}$~\cite{fu2018identifiability}, where $\Delta^{m\times r}=\{Y\in\R_+^{m\times r},e^\top Y=e^\top\}$ and $e$ is the all-one vector of appropriate dimension. 
% See~\Cref{minvolnmc:sec:idMinvolNMF} for more details on the identifiability of MinVol NMF. The constraint $W\in\Delta^{m\times r}$ ensures that the columns of $W$ 
% % \ngc{à définir; see above} 
% lie within the probabilistic simplex. The constraint $H^\top\in\Delta^{n\times r}$ can be seen as a budget assignment constraint: each feature should be used in the decomposition as much as the others. Both aforementioned constraints are without loss of generality relatively to NMF because of the scaling ambiguity between $W$ and $H$, that is, any NMF $(W,H)$ can be scaled so that $W\in\Delta^{m\times r}$ or $H^\top\in\Delta^{n\times r}$ is satisfied. 
% The constraint $H\in\Delta^{r\times n}$ is stronger than the other two as it is not without loss of generality relatively to NMF. For example, for the matrix  $X=\begin{pmatrix}
%     1 & 0 & 1\\
%     0 & 1 & 1
% \end{pmatrix} $, 
% there exists a rank-2 NMF of $X$ which is simply $X=IX$. However, any exact NMF of $X$ with the additional constraint that $H$ has to be column wise stochastic is of rank at least 3. Despite the loss of generality, this constraint remains useful in practice as it provides a soft clustering interpretation of the decomposition. It has been instrumental in hyperspectral imaging where each column of $H$ contains the abundances of the pure materials in a pixel which are nonnegative and sum to one~\cite{ma2014signal}. 
Among the three mentioned variants of MinVol, we will only consider the following formulation in the remainder of this chapter: 
%as it is the most ``neutral'': \ngc{neutral? why? expliquer qu'avec min-vol $H^\top\in\Delta^{n\times r}$ peut rendre $W$ mal conditionné et cela mène à des problèmes numériques? cf. notre article IEEE TSP}
%\begin{mini}
%	{\scriptstyle \substack{W\in\Delta^{m\times r},\\H\in\R_+^{r \times n}}}{\det(\Wt W )}{\label{minvolnmc:eq:exactminvol}}{}
%	\addConstraint{X}{=WH}{}
%\end{mini} 
\begin{mini}
	{\scriptstyle W,H}{\frac{1}{2}\|X-WH\|_F^2+\frac{\lambda}{2}\logdet(\Wt W +\delta I)}{\label{minvolnmc:eq:minvol}}{}
	\addConstraint{W\in\Delta^{m \times r}}{,~H\in\R_+^{r \times n},}{}
\end{mini}
where $\delta$ is a parameter that prevents the $\logdet$ from going to $-\infty$ when $W$ is rank deficient, and $\lambda\geq0$ balances the two terms. Note that the true volume spanned by the columns of $W$ and the origin is equal to $\frac{1}{r!}\sqrt{\det(\Wt W)}$, but minimizing $\logdet(\Wt W)$ is equivalent in the exact case and makes the problem numerically easier to solve because the function $\logdet(\cdot)$ is concave and it is easier to design a ``nice'' majorizer for it~\cite{fu2016robust}. 

\subsection{Identifiability of MinVol NMF}
\label{minvolnmc:sec:idMinvolNMF}

We say that $(W,H)$ is an exact MinVol NMF of size $r$ of $X$ if it solves 
\[
\min_{
W\in\Delta^{m \times r}, 
H\in\R_+^{r \times n}} \logdet(W^\top W) \text{ such that } X = WH. 
\] 
\begin{definition}[Essential uniqueness of MinVol NMF]
	The exact MinVol NMF $(W,H)$ of $X=WH$ of size $r$ is unique if, and only if, for any other exact MinVol NMF $(\tilde{W},\tilde{H})$ of $X=\tilde{W}\tilde{H}$ of size $r$, there exists a scaled permutation matrix $Q$ such that $\tilde{W}=WQ^{-1}$ and $\tilde{H}=QH$.
\end{definition}

Essential uniqueness is also referred as ``identifiability''. MinVol NMF with column wise simplex structured $H$ has first been proved to be identifiable in~\cite{fu2015blind}, under the so called sufficiently scattered conditions (SSC). 
\begin{definition}[SSC]  \label{minvolnmc:def:ssc}
	The matrix $H \in \mathbb{R}^{r \times n}_+$ is sufficiently scattered if the following two conditions are satisfied:\vspace{0.1cm}
	
	\noindent [SSC1]  $\mathcal{C} = \{x \in \R^r_+ \ | \ e^\top x \geq \sqrt{r-1} \|x\|_2 \} \; \subseteq \; \cone(H)$. \vspace{0.1cm}
	
	\noindent [SSC2]  There does not exist any orthogonal matrix $Q$ such that $\cone(H) \subseteq \cone(Q)$, except for permutation matrices. 
\end{definition}

These conditions require that the aperture of $\cone(H)$ is ``large enough'' by making sure $\cone(H)$ contains the second-order cone $\mathcal{C}$ which is tangent to every facet of the nonnegative orthant (SSC1), and not to tightly (SSC2). Geometrical interpretations of SSC1 is provided in~\cref{minvolnmc:fig:ssc_cone} and~\cref{minvolnmc:fig:scc_vs_notssc}, where $\Delta^{r}=\{y\in\R_+^{r},e^\top y=1\}$.


\begin{figure}
	\centering
	\input{minvolnmc/figures/ssc-cone.tex}
	\caption{Visualization of $\mathcal{C}$ with $r=3$. $e_i$'s are the canonical vectors.}
	\label{minvolnmc:fig:ssc_cone}
\end{figure}

\begin{figure}[htbp!]
\centering
	\input{minvolnmc/figures/ssc-vs-not-ssc.tex}
	\caption{Geometrical interpretation of SSC1 with $r=3$.}
	\label{minvolnmc:fig:scc_vs_notssc}
\end{figure}

Under the SSC, we have the following identifiability theorem. 
\begin{theorem}[\cite{leplat2019blind}]\label{minvolnmc:th:uniqueminvol}
	If $W\in\R^{m\times r}$ is full column rank and $H\in\R^{r\times n}$ satisfies the SSC, then the exact MinVol NMF of size $r$ of $X=WH$ is essentially unique. 
\end{theorem}

\Cref{minvolnmc:th:uniqueminvol} is fulfilled under relatively mild conditions, as the requirements are almost only on the factor $H$. The only assumption on $W$ is that it should be full rank. %\ngc{Tu essayes de donner le théorème le plus général possible... mais \cite{fu2015blind} c'est avec sum-to-one sur les colonnes de $H$... et tu n'as pas défini exact Minvol MF... Bref, je me contenterais de exact Minvol NMF qu'on a défini.}


\section{Nonnegative matrix completion (NMC)}
\label{minvolnmc:sec:NMC}

In this section, we justify the choice of the minimum-volume criterion for the task of nonnegative matrix completion. Matrix completion in general has been well studied, especially by the compressed sensing community. Among the techniques to perform matrix completion, the low-rank approach often arises, because the low-rank structure has been observed to be quite powerful in this setting, as it is able to identify hidden (linear) features in data. However, minimizing the rank of the estimation matrix while guaranteeing the equality constraints on the set of observed entries is NP-hard in general. 
A good convex relaxation that promotes low-rank structures is the nuclear norm minimization; see~\cite{recht2010guaranteed}. This is coming from the fact that the rank is the $\ell_0$ norm of the vector of the singular values, while the nuclear norm is the $\ell_1$ norm of this vector. Still, this requires to store the whole estimation $\tilde{X}$ of $X$, and it also becomes harder to impose additional structuring constraints. When the rank is known, we can fully exploit the low-rank structure by working with the low-rank factors $W$ and $H$ instead. It is then easier to add some structuring constraints on $W$ and $H$. Also, this allows one to deal with larger problems. 
Since 
$$
\|X\|_* = \min_{X=WH}\frac{1}{2}\left(\|W\|_F^2+\|H\|_F^2\right),
$$ 
\sloppy a good alternative to the nuclear norm regularization is then the regularizer $\frac{1}{2}\left(\|W\|_F^2+\|H\|_F^2\right)$~\cite{srebro2005maximum}. 
If the rank is unknown, an overestimated rank coupled with a proper penalization of $\frac{1}{2}\left(\|W\|_F^2+\|H\|_F^2\right)$ can yield state-of-the-art results. For example, in~\cite{rendle2022revisiting}, a properly tuned matrix factorization model using the above regularizer can outperform deep neural networks on recommendation systems. 
In~\cite{liu2017newtheory}, they showed that the sightly different regularizer $\|W\|_*+\frac{1}{2}\|H\|^2_F$ yields better results than $\frac{1}{2}\left(\|W\|_F^2+\|H\|_F^2\right)$, both with uniform or non-uniform samplings. Going back to our point of interest, it is interesting to observe that the MinVol regularizer provides more adaptability as a (non-convex) relaxation of the rank~\cite{leplat2019minimum}, since 
$\logdet(W^\top W+\delta I) = \sum_i\log(\sigma_i^2(W)+\delta).$ 
\begin{figure}[htb!]
\centering
\begin{tikzpicture}
	\begin{axis}[
		xmin=0, xmax=1.5, % x scale
		ymin=0, ymax=1.25, % y scale
		domain=0:1.5,  % added, key improvements
		legend pos=south east,
		width=\textwidth,
		height=6cm,
		]
		\addplot    {x};
		\addlegendentry{$\ell_1$}
		\addplot    {(ln(x^2+0.1)-ln(0.1))/(ln(1+0.1)-ln(0.1))};
		\addlegendentry{$f_{10^{-1}}(x)$}
		\addplot    {(ln(x^2+1e-3)-ln(1e-3))/(ln(1+1e-3)-ln(1e-3))};
		\addlegendentry{$f_{10^{-3}}(x)$}
		\addplot    {(ln(x^2+1e-6)-ln(1e-6))/(ln(1+1e-6)-ln(1e-6))};
		\addlegendentry{$f_{10^{-6}}(x)$}
		\addplot    {(ln(x^2+1e-9)-ln(1e-9))/(ln(1+1e-9)-ln(1e-9))};
		\addlegendentry{$f_{10^{-9}}(x)$}
		\addplot[only marks] 	{min(x*1e9,1)};
		\addlegendentry{$\ell_0$}
	\end{axis}
\end{tikzpicture}
\caption{Function $f_\delta(x)=\frac{\ln(x^2+\delta)-\ln(\delta)}{\ln(1+\delta)-\ln(\delta)}$ for various values of $\delta$, along the $\ell_0$ and $\ell_1$ norm.}
\label{minvolnmc:fig:minvolL0L1}
\end{figure}
As it can be seen in~\cref{minvolnmc:fig:minvolL0L1}, $\logdet(W^\top W + \delta I)$ approximates a range of behaviors between the $\ell_0$ and the $\ell_1$ norms. In particular, as $\delta$ goes to zero, $\logdet(W^\top W + \delta I)$ converges to the $\ell_0$ norm of the vector of singular values of $X$, up to a constant factor.  Hence the MinVol criterion $\logdet(W^\top W+\delta I)$ is clearly a good candidate as a regularizer for NMC. 

Let us now propose two models to tackle NMC. 
The first one is to adapt~\eqref{minvolnmc:eq:minvol} to the NMC problem, which yields
\begin{mini}
	{\scriptstyle W,H}{\frac{1}{2}\|\P_\Omega(X-WH)\|_F^2+\frac{\lambda}{2}\logdet(\Wt W +\delta I)}{\label{minvolnmc:eq:minvolcompletion}}{}
	\addConstraint{W\in\Delta^{m \times r}}{,~H\in\R_+^{r \times n}.}{}
\end{mini} 
\Cref{minvolnmc:th:uniqueminvol} does not extend to the case where some values are missing. If the matrix completion is not unique, then it is impossible to guarantee a unique recovery of the matrices $W$ and $H$. Hence, a trivial way to adapt~\Cref{minvolnmc:th:uniqueminvol} to missing values is to add the condition that matrix completion under MinVol should be unique. However, conditions under which solving~\eqref{minvolnmc:eq:minvolcompletion} recovers a unique completion are, up to now, unknown.

The second one introduces a new variant of MinVol NMF which is not simplex structured. Inspired by the regularizer $\|W\|_*+\frac{1}{2}\|H\|^2_F$ and motivated by the link between the behavior of the nuclear norm and the MinVol criterion, here we consider $\logdet(W^\top W+\delta I)+\|H\|^2_F$ as a regularizer. The resulting new MinVol NMF adapted for NMC is 
\begin{align}
   \min_{W,H} & \frac{1}{2}\|\P_\Omega(X\text{$-$}WH)\|_F^2+\frac{\lambda}{2}\logdet(\Wt W\text{$+$}\delta I)+\frac{\gamma}{2}\|H\|_F^2 \nonumber \\  
   & \text{ s.t. }  W\in\R_+^{m \times r} ,~H\in\R_+^{r \times n}. \label{minvolnmc:eq:newminvol} 
\end{align} 
% \begin{mini}
% 	{\scriptstyle W,H}{\frac{1}{2}\|\P_\Omega(X-WH)\|_F^2+\frac{\lambda}{2}\logdet(\Wt W +\delta I)+\frac{\gamma}{2}\|H\|_F^2}{\label{minvolnmc:eq:newminvol}}{}
% 	% \breakObjective{+\frac{\gamma}{2}\|H\|_F^2}
% 	\addConstraint{W\in\R_+^{m \times r}}{,~H\in\R_+^{r \times n},}{}
% \end{mini} 
where $\lambda\geq0$ and $\gamma\geq0$ balance the regularizers.
Note that neither $W$ nor $H$ is simplex structured. The scaling ambiguity coupled with the volume penalization is counter balanced by the penalization of $\|H\|_F^2$. In fact, in the exact case and when $\delta=0$, every row of $H$ has the same norm at optimality. Consider a feasible $(W,H)$ for~\eqref{minvolnmc:eq:newminvol} such that $X=WH$ and let ${f(D)=\frac{\lambda}{2}\logdet(D^{-1}W^\top WD^{-1})+\frac{\gamma}{2}\|DH\|_F^2}$ where $D=\diag(d_1,\dots,d_r)$ is a positive diagonal matrix that can be seen as the scaling ambiguity between $W$ and $H$. Nullifying the gradient of $f$ relatively to each $d_i$, we have that $d_i^2=\frac{\lambda}{\gamma\|H(i,:)\|_F^2}$, meaning that at optimality $\|H(i,:)\|_F^2=\frac{\lambda}{\gamma}$ for all $i$. 



% \ngc{mentionner identifiability pour completion unique?} 

%\ngc{mentionner le lemme égalité des normes lignes de H à l'optimalité dans le cas exact?}

\section{Algorithms}
\label{minvolnmc:sec:algorithms}

In~\Cref{minvolnmc:sec:exp}, we compare NMF, MinVol~\eqref{minvolnmc:eq:minvolcompletion} and new MinVol~\eqref{minvolnmc:eq:newminvol}. For a fair comparison, these models are fit with the same algorithmic scheme, adapted from~\cite{vuthanh2021inertial}, which is an extrapolated alternating block majorization-minimization method. Our adaptation is described in~\Cref{minvolnmc:alg:generictitan}, where $\P_{\Delta^{m\times r}}$ (respectively $\P_{\R_+^{m\times r}}$)  projects a matrix of size $m\times r$ onto $\Delta^{m\times r}$ (respectively $\R_+^{m\times r}$). See~\cite{condat2016fast} for the details on the projection onto $\Delta^{m\times r}$. Essentially, the updates for $W$ and $H$ are several projected gradient descent steps, performed with a step size equal to the inverse of the Lipschitz constant. The updates for each model and each factor, as well as the corresponding Lipschitz constant, are given in~\Cref{minvolnmc:tab:updatesW} and~\Cref{minvolnmc:tab:updatesH}. The used Lipschitz constants are deliberately not tight. Consider the MinVol NMF update of $H$ for instance. 
% Assuming, that $W$ is fixed, updating $H$ consists in solving
% \begin{align*}
% & \argmin_{H\geq0}\frac{1}{2}\|\P_\Omega(X-WH)\|_F^2+\frac{\lambda}{2}\logdet(\Wt W +\delta I)\\
% = & \argmin_{H\geq0}\frac{1}{2}\|\P_\Omega(X-WH)\|_F^2 :=f(H).
% \end{align*}
Let $M\in\{0,1\}^{m\times n}$ be such that $M(i,j)=1$ if $(i,j)\in\Omega$, $M(i,j) = 0$ otherwise. A tighter Lipschitz constant is $\max_j \left\|W^\top((M(:,j)e^\top)\circ W)\right\|_2$.
% $$
% 	\left\|\frac{\partial f}{\partial H}(H_1)-\frac{\partial f}{\partial H}(H_1)\right\|^2_F = \left\|W^\top\P_\Omega(WH_1-WH_2)\right\|^2_F
% $$
% \begin{align*}
% 	&= \sum_j \left\|W^\top(M(:,j)\circ(W(H_1(:,j)-H_2(:,j))))\right\|^2_F\\
% 	&\leq \sum_j \left\|W^\top((M(:,j)e^\top)\circ W)\right\|^2_2 \left\|H_1(:,j)-H_2(:,j)\right\|^2_F\\
% 	&\leq \max_j \left\|W^\top((M(:,j)e^\top)\circ W)\right\|^2_2 \left\|H_1-H_2\right\|^2_F.\\
% \end{align*}
% A tighter Lipschitz constant than $\|W^\top W\|_2$ would then be $\max_j \left\|W^\top((M(:,j)e^\top)\circ W)\right\|_2$. 
We deliberately keep $\|W^\top W\|_2$ as it is less costly to compute and the additional cost might not be worth it. Moreover, if at least one column of $X$ is fully observed, then ${\max_j \left\|W^\top((M(:,j)e^\top)\circ W)\right\|_2 = \|W^\top W\|_2} = \|W\|_2^2$. 

\begin{algorithm}[htb!]
\caption{Main algorithm scheme}
\label{minvolnmc:alg:generictitan}
\SetKwInOut{Input}{input}
\DontPrintSemicolon
\Input{data matrix $X \in \mathbb{R}^{m \times n}$, initial factors $W \in \R_+^{m \times r}$  and $H\in \R_+^{r \times n}$}
$\alpha_1=\alpha_2=1,~\Wold=W,~\Hold=H$\;
\While{stopping criteria not satisfied\label{minvolnmc:line:whileouterloop}}{
	\While{stopping criteria not satisfied\label{minvolnmc:line:whileW}}{
		$\alpha_0=\alpha_1,\quad\alpha_1=\frac{1}{2}(1+\sqrt{1+4\alpha_0^2})$\;
		% $\alpha_1=\frac{1}{2}(1+\sqrt{1+4\alpha_0^2})$\;
		% $\beta=\frac{\alpha_0-1}{\alpha_1}$\;
		$\Wextra=W+\frac{\alpha_0-1}{\alpha_1}(W-\Wold)$\;
		$\Wold=W$\;
		Update $W$ according to~\Cref{minvolnmc:tab:updatesW}\;
	}
	\While{stopping criteria not satisfied\label{minvolnmc:line:whileH}}{
		$\alpha_0=\alpha_2,\quad\alpha_2=\frac{1}{2}(1+\sqrt{1+4\alpha_0^2})$\;
		% $\alpha_2=\frac{1}{2}(1+\sqrt{1+4\alpha_0^2})$\;
		% $\beta=\frac{\alpha_0-1}{\alpha_2}$\;
		$\Hextra=H+\frac{\alpha_0-1}{\alpha_2}(H-\Hold)$\;
		$\Hold=H$\;
		Update $H$ according to~\Cref{minvolnmc:tab:updatesH}\;
	}
}
\end{algorithm}
\begin{table}[htb!]
	\centering
	\begin{tabular}{c||c}
		& Update \\ \hline &  \\
		MinVol & $\P_{\Delta^{m\times r}}\left(\Wextra-\frac{1}{L}\nabla_W\right)$ \\ &\\ \hline &  \\
		new MinVol~/~NMF (with $\lambda=0$) &  $\P_{\R_+^{m\times r}}\left(\Wextra-\frac{1}{L}\nabla_W\right)$
	\end{tabular}
\caption{Updates for $W$ according to the model, where $P=(\Wextra^\top\Wextra+\delta I)^{-1}$, $L=\|HH^\top+\lambda P\|_2$ and ${\nabla_W=\P_\Omega\left(\Wextra H-X\right)H^\top+\lambda WP}$.}
\label{minvolnmc:tab:updatesW}
\end{table}
\begin{table}[hbt!]
	\centering
	\begin{tabular}{c||c|c}
		& $L$ & Update \\ \hline & & \\
		MinVol~/~NMF & $\|W^\top W\|_2$ & $\P_{\R_+^{r\times n}}\left(\Hextra-\frac{1}{L}\nabla_H\right)$ \\ &&\\ \hline & & \\
		new MinVol & $\|W^\top W+\gamma I\|_2$ & $\P_{\R_+^{r\times n}}\left(\frac{L-\gamma}{L}\Hextra-\frac{1}{L}\nabla_H\right)$
	\end{tabular}
	\caption{Updates for $H$ according to the model, where $\nabla_H=W^\top\P_\Omega\left(W\Hextra-X\right)$.}
	\label{minvolnmc:tab:updatesH}
\end{table}

%\ovt{All algorithms have the same computational complexity, with vanilla MinVol being slightly more expensive in practice due to the projection $\P_{\Delta^{m\times r}}(.)$, which is in $O(rm\log(m)$ without multi-threading.}

\section{Experiments}
\label{minvolnmc:sec:exp}

The goal of this section is to highlight the performance of the MinVol criterion for NMC. 
All experiments are run with Julia on a PC with an Intel(R) Core(TM) i7-9750H CPU @ 2.60GHz and 16GB RAM. All displayed measurements are averaged out of 20 runs. The code is available at \url{https://gitlab.com/vuthanho/minvol-nmc}. 
% The compared models are NMF, MinVol with $\lambda=1$, MinVol with $\lambda=1$ and automatic tuning as in~\cite{nguyen2023towards}, and the new proposed MinVol with $\lambda=1$, $\gamma=0.01$ and automatic tuning for $\lambda$ and $\gamma$. The automatic tuning is triggered when the difference between the current and the last objective values divided by $\|\P_\Omega(X)\|_F^2$ is less than $10^{-3}$. The results of NMF are here to provide a baseline of a non-regularized model. As in~\cite{leplat2019minimum}, the values of $\lambda$ and $\gamma$ are rescaled relatively to the initial reconstruction error, that is
% \begin{align*}
% 	\lambda~\leftarrow~&\lambda\frac{\max(\|\P_\Omega(X-W_0H_0)\|_F^2,10^{-6})}{|\logdet(W_0^\top W_0+\delta I)|},\\
% 	\gamma~\leftarrow~&\gamma\frac{\max(\|\P_\Omega(X-W_0H_0)\|_F^2,10^{-6})}{\|H_0\|_F^2}.
% \end{align*}
% All models are given 20 inner and 50 outer iterations. All models are also initialized with the same warm start, which is the output of 500 iterations of NMF where the columns of $W$ are simplex-structured. 
% \ngc{d'abord parler des algo, ensuite $\lambda$ et $\gamma$ et ensuite automatic tuning?} \ngc{aussi parler de l'initialisation $(W_0,H_0)$?} 
The compared models are NMF (to provide a baseline of a non-regularized model), MinVol~\eqref{minvolnmc:eq:minvolcompletion}, and the new proposed MinVol~\eqref{minvolnmc:eq:newminvol}. For all models, the stopping criteria of the \textbf{while} loop in~\cref{minvolnmc:line:whileouterloop} is just a number of outer iterations equal to 50, and the stopping criteria of the two \textbf{while} loops in~\cref{minvolnmc:line:whileW,minvolnmc:line:whileH} is a number of inner iterations equal to 20.
%All models are given 20 inner and 50 outer iterations. 
All models are also initialized with the same warm start $(W_0,H_0)$, which is the output of 500 iterations of NMF where the columns of $W$ are simplex-structured. In this setting, all methods converge. For both MinVols, $\lambda$ is first set to $\frac{\max(\|\P_\Omega(X-W_0H_0)\|_F^2,10^{-6})}{|\logdet(W_0^\top W_0+\delta I)|}$. For the new proposed MinVol, $\gamma$ is first set to $0.01\frac{\max(\|\P_\Omega(X-W_0H_0)\|_F^2,10^{-6})}{\|H_0\|_F^2}$. On the hyperparameters $\lambda$ and $\gamma$, we adapt the automatic tuning method developed in~\cite{nguyen2023towards}. The automatic tuning does not introduce a significant additional cost and is triggered when the difference between the current and the last objective values divided by $\|\P_\Omega(X)\|_F^2$ is less than $10^{-3}$. 

\paragraph{First experiment: noiseless synthetic data} 
The first experiment focuses on both data completion and recovery of the exact generating factors in a noiseless case. For this experiment, for a given rank $r$, we randomly generate two factors $(W,H)=[0,1]^{200\times r}\times[0,1]^{r\times200}$ following a uniform distribution. Then, $80\%$ random values of $H$ are set to zeros. This is a reasonable assumption in real scenarios such as hyperspectral unmixing. For the explored range of ranks, this will provide almost surely a sufficiently scattered $H$. Then, we generate the full data matrix $X$ simply by computing $WH$. The average of the elements of $X$ is always set to 1, dividing $X$ by its average. Finally, we create the observed data $\tilde{X}$ by removing a certain percentage of the entries in $X$. We vary the rank from 5 to 10, and the percentage of missing values from 80\% to 90\%. We report the root-mean-squared error (RMSE) of the missing values according to~\cref{minvolnmc:def:rmse} and the maximum subspace angle between the factor $W$ that took part in generating the data $X$ and its estimation $\tilde{W}$ according to~\cref{minvolnmc:def:angle}.
 \begin{definition}[RMSE]
 	\label{minvolnmc:def:rmse}
 	The RMSE on the unobserved set $\overbar{\Omega}$ is defined as follows \\$${\text{RMSE}(\tilde{X},WH)=\sqrt{\frac{1}{|\overbar{\Omega}|} \| \P_{\overbar{\Omega}} (\tilde{X}-WH)\|^2_F}.}$$
 	% $$\text{RMSE}(\tilde{X},WH)=\sqrt{\frac{1}{|\overbar{\Omega}|} \| \P_{\overbar{\Omega}} (\tilde{X}-WH)\|^2_F}.$$
 \end{definition}
 \begin{definition}[Subspace angle] 
 	\label{minvolnmc:def:angle}
 	Let $USV$ and $\tilde{U}\tilde{S}\tilde{V}$ respectively be the singular value decomposition of $W$ and $\tilde{W}$. Then the angle between the two subspaces specified by the columns of $W$ and $\tilde{W}$ is defined as follows
 	$$\text{Angle}(W,\tilde{W})=\arcsin(\min(1,\|\tilde{U} - UU^\top\tilde{U}\|_ 2)).$$ 
 \end{definition} 
 The RMSEs are reported in~\cref{minvolnmc:fig:noiseless_rmse} and the subspace angles in~\cref{minvolnmc:fig:noiseless_angle}. MinVol NMF coupled with the proposed auto-tuning proposed in~\cite{nguyen2023towards} clearly outperforms the vanilla MinVol NMF with a fixed $\lambda$. The auto-tuned MinVol NMF is itself outperformed by our new proposed variant of MinVol NMF. For $90\%$ missing values and a rank equal to 10 for instance, the average RMSE of the auto-tuned Minvol is 0.52 while it is 0.41 for the new MinVol.% \ngc{un peu quantifier?} 
 
 
\paragraph{Second experiment: noisy synthetic data} We keep the same settings as in the first experiment, while fixing the rank to 10, and adding some uniformly distributed noise. The noise level corresponds to the RMSE between the clean data and the noisy data. We vary the noise level from 0 to 1 and the percentage of missing values from $80\%$ to $90\%$. We report the RMSE in~\cref{minvolnmc:fig:noisy_rmse}. It is not necessary to report the subspace angle since it is degrading too fast. Perfect matrix completion is a necessary condition to retrieve a low subspace angle, which is already not possible starting from a noise level equal to 0.2. Results in~\cref{minvolnmc:fig:noisy_rmse} show that our proposed variant of MinVol NMF is more consistent relatively to the percentage of missing values and more precise than vanilla MinVol NMF in the presence of noise.

\def\step{0.35}
\def\nwidth{11}
\def\nheight{6}
\def\maxrmse{1}

\begin{figure}[htbp!]
	\centering
    \begin{subfigure}{0.45\textwidth}
	\centering
    \caption{NMF}\vspace{-0.35cm}
        \input{minvolnmc/figures/angle_NMF.tex}
    \end{subfigure}
	\hspace{0.5cm}
    \begin{subfigure}{0.45\textwidth}
	\centering
    \caption{MinVol}\vspace{-0.35cm}
        \input{minvolnmc/figures/angle_Minvol.tex}
    \end{subfigure}

    \begin{subfigure}{0.45\textwidth}
	\centering
    \caption{auto MinVol}\vspace{-0.35cm}
        \input{minvolnmc/figures/angle_auto_Minvol.tex}
    \end{subfigure}
	\hspace{0.5cm}
    \begin{subfigure}{0.45\textwidth}
	\centering
    \caption{new MinVol}\vspace{-0.35cm}
        \input{minvolnmc/figures/angle_new_Minvol.tex}
    \end{subfigure}
\caption{Average angle according to the rank $r$ and to the percentage of missing values over 20 runs.}
\label{minvolnmc:fig:noiseless_angle}
\end{figure}


\begin{figure}[htbp!]
\centering
	\begin{subfigure}{0.45\textwidth}
	\centering
	\caption{NMF}
		\input{minvolnmc/figures/rmse_NMF.tex}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.45\textwidth}
	\centering
	\caption{MinVol}
		\input{minvolnmc/figures/rmse_Minvol.tex}
	\end{subfigure}

	\begin{subfigure}{0.45\textwidth}
	\centering
	\caption{auto MinVol}
		\input{minvolnmc/figures/rmse_auto_Minvol.tex}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.45\textwidth}
	\centering
	\caption{new MinVol}
		\input{minvolnmc/figures/rmse_new_Minvol.tex}
	\end{subfigure}
\caption{Average RMSE according to the rank $r$ and to the percentage of missing values over 20 runs.}
\label{minvolnmc:fig:noiseless_rmse}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\begin{subfigure}{0.45\textwidth}
		\centering
		\caption{NMF}\vspace{-0.35cm}
		\input{minvolnmc/figures/noisy_rmse_NMF.tex}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.45\textwidth}
		\centering
		\caption{MinVol}\vspace{-0.35cm}
		\input{minvolnmc/figures/noisy_rmse_Minvol.tex}
	\end{subfigure}

	\begin{subfigure}{0.45\textwidth}
		\centering
		\caption{auto MinVol}\vspace{-0.35cm}
		\input{minvolnmc/figures/noisy_rmse_auto_Minvol.tex}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.45\textwidth}
        \centering
        \caption{new MinVol}\vspace{-0.35cm}
        \input{minvolnmc/figures/noisy_rmse_new_Minvol.tex}
	\end{subfigure}
\caption{Average RMSE according to the noise level and to the percentage of missing values over 20 runs.}
\label{minvolnmc:fig:noisy_rmse}
\end{figure}


% \begin{figure*}[htbp!]
% \centering
% \begin{subfigure}{0.4\textwidth}
% \centering
% \caption{NMF}
%     \input{minvolnmc/figures/rmse_NMF.tex}
% \end{subfigure}
% \begin{subfigure}{0.4\textwidth}
% \centering
% \caption{MinVol}
%     \input{minvolnmc/figures/rmse_Minvol.tex}
% \end{subfigure}

% \begin{subfigure}{0.4\textwidth}
% \centering
% \caption{auto MinVol}
%     \input{minvolnmc/figures/rmse_auto_Minvol.tex}
% \end{subfigure}
% \begin{subfigure}{0.4\textwidth}
% \centering
% \caption{new MinVol}\vspace{-0.25cm}
% \input{minvolnmc/figures/rmse_new_Minvol.tex}
% \end{subfigure}
% \caption{Average RMSE according to the rank $r$ and to the percentage of missing values over 20 runs.}
% \label{minvolnmc:fig:noiseless_rmse}
% \end{figure*}

% \begin{figure*}[htbp!]
% \centering
% \begin{subfigure}{0.24\textwidth}
% \centering
% \caption{NMF}
%     \input{minvolnmc/figures/angle_NMF.tex}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \centering
% \caption{MinVol}
%     \input{minvolnmc/figures/angle_Minvol.tex}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \centering
% \caption{auto MinVol}
%     \input{minvolnmc/figures/angle_auto_Minvol.tex}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \centering
% \caption{new MinVol}\vspace{-0.25cm}
% \input{minvolnmc/figures/angle_new_Minvol.tex}
% \end{subfigure}
% \caption{Average angle according to the rank $r$ and to the percentage of missing values over 20 runs.}
% \label{minvolnmc:fig:noiseless_angle}
% \end{figure*}
    
% \begin{figure*}[htbp!]
% 	\def\step{0.3}
% 	\def\nwidth{11}
% 	\def\nheight{6}
% 	\def\maxrmse{1}
% 	\centering
% 	\begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\caption{NMF}
% 		\input{minvolnmc/figures/noisy_rmse_NMF.tex}
% 	\end{subfigure}
% 	\begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\caption{MinVol}
% 		\input{minvolnmc/figures/noisy_rmse_Minvol.tex}
% 	\end{subfigure}
% 	\begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\caption{auto MinVol}
% 		\input{minvolnmc/figures/noisy_rmse_auto_Minvol.tex}
% 	\end{subfigure}
% 	\begin{subfigure}{0.24\textwidth}
% 	\centering
% 	\caption{new MinVol}\vspace{-0.25cm}
% 	\input{minvolnmc/figures/noisy_rmse_new_Minvol.tex}
% 	\end{subfigure}
% 	\caption{Average RMSE according to the noise level and to the percentage of missing values over 20 runs.}
% 	\label{minvolnmc:fig:noisy_rmse}
% \end{figure*}

\section{Conclusion and Discussion}
\label{minvolnmc:sec:conclusion}

This chapter argued on the favor of using more the MinVol criterion in the domain of matrix completion, which has never been explored before. Not only the MinVol criterion can emulate a broad of behaviors going from the rank minimization to the nuclear minimization, but it also acts in favor of recovering the unique decomposition of a low-rank matrix if it exists. This chapter also introduced a new variant of MinVol NMF which is not simplex-structured. Experiments show that a properly tuned MinVol NMF provides encouraging results, both on the task of matrix completion and unique factors recovery. Last but not least, experiments show that our new proposed variant of MinVol NMF outperforms vanilla MinVol NMF. Future work will focus on the potential identifiability of this new variant and on comparing with other matrix completion algorithms.

==> polytopicmf/figures/old-pmfssc1notsatisfied.tex <==
\tdplotsetmaincoords{80}{10}
%\tdplotsetmaincoords{45}{135}
%z={(0,1)},y={(0.4,0.4)},x={(1,0)}
\begin{tikzpicture}[scale=2.7,tdplot_main_coords,axis/.style={->,dashed},thick,curve/.style={red,densely dotted,thick}]
	
	\coordinate  (A) at (0,0,1){};
	\coordinate  (B) at (1,0,1){};
	\coordinate  (C) at (1,0,0){};
	\coordinate  (D) at (0,0,0){};
	\coordinate  (E) at (0,1,1){};
	\coordinate  (F) at (1,1,1){};
	\coordinate  (G) at (1,1,0){};
	\coordinate  (H) at (0,1,0){};
	
	\coordinate  (a) at (0.8,0.2,0){};
	\coordinate  (b) at (0,0.8,0.2){};
	\coordinate  (c) at (0.2,0,0.8){};
	\coordinate  (d) at (0.2,1,0.8){};
	\coordinate  (e) at (0.8,0.2,1){};
	\coordinate  (f) at (1,0.8,0.2){};
	
	% Probabilistic simplex
	\draw [red] (A) -- (C) -- (H) -- cycle;
	% Back of hypercube
	\draw [orange,dashed] (G) -- (H) -- (E);
	\draw [orange,dashed] (H) -- (D);
	
	
	% -- remove these 3 lines if no axis is preferred
%	\draw[axis] (0, 0, 0) -- (1.2, 0, 0) node [right] {};
%	\draw[axis] (0, 0, 0) -- (0, 1.2, 0) node [above] {};
%	\draw[axis] (0, 0, 0) -- (0, 0, 1.2) node [above] {};
	
	% draw ball
	
	\coordinate (O) at (0.5,0.5,0.5);
	
	\foreach \angle in {-90,0,90}
	{
		%calculate the sine and cosine of the angle
		\tdplotsinandcos{\sintheta}{\costheta}{\angle}%
		
		%define a point along the z-axis through which to draw
		%a circle in the xy-plane
		\coordinate (P) at (0.5,0.5,0.5+\sintheta/2);
		
		%draw the circle in the main frame
		\tdplotdrawarc[curve,blue]{(P)}{\costheta/2}{0}{360}{}{}
		
		%define the rotated coordinate frame based on the angle
		\tdplotsetthetaplanecoords{\angle}
		
		%draw the circle in the rotated frame
		\tdplotdrawarc[curve,blue,tdplot_rotated_coords]{(O)}{0.5}{0}{360}{}{}
	}
	
	
	% fill gray color with opacity
	\fill[gray!50,opacity=0.2] (a) -- (b) -- (c)-- cycle; 
	\fill[gray!50,opacity=0.2] (a) -- (e) -- (c)-- cycle; 
	\fill[gray!50,opacity=0.2] (a) -- (b) -- (f)-- cycle;
	\fill[gray!50,opacity=0.2] (a) -- (e) -- (f)-- cycle;
	\fill[gray!50,opacity=0.2] (d) -- (c) -- (e)-- cycle; 
	\fill[gray!50,opacity=0.2] (d) -- (b) -- (f)-- cycle; 
	\fill[gray!50,opacity=0.2] (d) -- (e) -- (f)-- cycle;
	\fill[gray!50,opacity=0.2] (d) -- (c) -- (b)-- cycle;
	% draw frames
	\draw [] (a) -- (e) -- (c)-- cycle;
	\draw [] (a) -- (e) -- (f)-- cycle;
	\draw [] (a) -- (b) -- (c)-- cycle;
	\draw [] (d) -- (e) -- (c)-- cycle;
	\draw [dashed] (d) -- (b) -- (f)-- cycle;
	
	\foreach \i in {a,b,c,d,e,f}
	{
		\draw[fill=black] (\i) circle (0.05em)
		node[above right] {};
	}
	
	\draw [orange] (A) -- (B) -- (C) -- (D) -- cycle;
	\draw [orange] (A) -- (E) -- (F) -- (B);
	\draw [orange] (F) -- (G) -- (C);
	\draw [red] (A) -- (C);
\begin{axis}[legend style={nodes={scale=0.3, transform shape}},
legend image post style={scale=0.3},
legend style={at={(0,0)},
anchor=south west},
axis lines=none,
width=2cm,
height=2cm,
xmin=0,xmax=1,ymin=0,ymax=1
]
\addplot [red,line width=2pt,forget plot]
		coordinates{
			(0,1)};
\addlegendimage{color=red,line width=2pt}
\addlegendimage{color=black,
mark=*,mark options={solid},only marks}
\addlegendimage{line width=2pt,blue,dashed}

% \legend{$\Delta^3$,$W^\top$,$\conv(W^\top)$,$\E_{[0,1]^3}$,${[0,1]^3}$}
\legend{$\Delta^3$,$W^\top$,$\E_{[0,1]^3}$}
\end{axis}
\end{tikzpicture}

==> randspa/code-randspa.tex <==
\begin{algorithm}[htb!]
\caption{Randomized Successive Projection Algorithm (RandSPA) \label{algo:randspa}}

\KwIn{The matrix $X \in \mathbb{R}^{m \times n}$, the number~$r$ of columns to extract, the rank $p$ of $R$, the conditioning $\kappa$.}

\KwOut{Index set $\mathcal{J}$ of cardinality $r$ such that $X \approx X(:,\mathcal{J}) H$ for some $H \geq 0$.}

Let $\mathcal{J} = \emptyset$, $P^\bot = I_m$, $V = [\;]$. \\

\For{$k=1$ : $r$}
{
    Let $R\in\mathbb{R}^{m\times p}$ be a random set of vectors mutually orthogonal such that $\|R(:,j)\|_2^2=\kappa - (j-1)\frac{\kappa-1}{p-1}$ for all $j$.\\
    Let $j_k = \argmax_{1 \leq j \leq n} \|R^{\top}P^{\bot}X(:,j)\|$. (Break ties arbitrarily, if necessary.)\\
    Let $\mathcal{J} = \mathcal{J} \cup \{ j_k  \}$. \\
    
    Update the projector $P^\bot$ onto the orthogonal complement of $W = X(:,\mathcal{J})$:
    \begin{align*}
    & v_k = \frac{P^\bot X(:,j_k)}{\| P^\bot X(:,j_k) \|_2},\\
    & V = [V \, v_k],\\
    & P^\bot \leftarrow \left( I_m - VV^T \right).
    \end{align*}
}
\end{algorithm}

